Constraining braneworlds with entanglement entropy

We propose swampland criteria for braneworlds viewed as effective field theories of defects coupled to semiclassical gravity. We do this by exploiting their holographic interpretation. We focus on general features of entanglement entropies and their holographic calculations. Entropies have to be positive. Furthermore, causality imposes certain constraints on the surfaces that are used holographically to compute them, most notably a property known as causal wedge inclusion. As a test case, we explicitly constrain the Dvali--Gabadadze--Porrati term as a second-order-in-derivatives correction to the Randall--Sundrum action. We conclude by discussing the implications of these criteria for the question on whether entanglement islands in theories with massless gravitons are possible in Karch--Randall braneworlds.

==> figs/planarBH.tex <==
\begin{figure}
\centering
\begin{tikzpicture}
%\node at (4,2) {};
\draw[-,draw=none,fill=black!10] (-6,0) to (0,0) to (-6,2) -- cycle;
\draw[-,draw=none,fill=black!10] (3,0) to (0,0) to (3,2) -- cycle;

\draw[-] (-1.75,0) arc (180:161.5:1.75);
\draw[-] (1.1,0) arc (0:33.5:1.1);

\draw[-,black!20] (-6,0) to (3,0);

\draw[-,thick,red] (0,0) to (-6,2);
\draw[-,thick,red] (0,0) to (3,2);

%\draw[-,thick,black!20!green] (0,0) to (-2,0.667);
%\draw[-,thick,red] (-2,0.667) to (-3,1);
%\draw[-,thick,black!20!green] (0,0) to (3/1.7,2/1.7);
%\draw[-,thick,red] (3/1.7,2/1.7) to (3,2);

\node[red] at (0,0) {$\bullet$};
\node at (0,0) {$\circ$};


\node at (0.8,0.2) {$\theta_1$};
\node at (-1.4,0.2) {$\theta_2$};




\draw[-,dashed] (-6,2) to (3,2);

\draw[->] (0,0.8) to (0,1.75);
\draw[->] (-0.2,1) to (0.75,1);
\node at (0.75,1.25) {$y$};
\node at (-0.25,1.75) {$z$};
\end{tikzpicture}
\caption{A fixed-$t$, fixed-$\vec{x}$ slice of a planar AdS-Schwarzschild geometry consisting of two planar branes (in red), each at a fixed angle $\theta_1,\theta_2 \in \left(0,\frac{\pi}{2}\right)$ with respect to the conformal boundary. The defect (the red point) is at $y = z = 0$ and the horizon (the dashed line) is at $z = z_{\text{h}}$. While this setup is geometrically simple to write down, it is not a solution to the RS equations. In particular, the branes are not surfaces of constant extrinsic curvature, and so they do not satisfy \eqref{bdryEOMRS}.}
\label{figs:planarBH}
\end{figure}
